Toward Joint Language Modeling for Speech Units and Text

Speech and text are two major forms of human language. The research community has been focusing on mapping speech to text or vice versa for many years. However, in the field of language modeling, very little effort has been made to model them jointly. In light of this, we explore joint language modeling for speech units and text. Specifically, we compare different speech tokenizers to transform continuous speech signals into discrete units and use different methods to construct mixed speech-text data. We introduce automatic metrics to evaluate how well the joint LM mixes speech and text. We also fine-tune the LM on downstream spoken language understanding (SLU) tasks with different modalities (speech or text) and test its performance to assess the model's learning of shared representations. Our results show that by mixing speech units and text with our proposed mixing techniques, the joint LM improves over a speech-only baseline on SLU tasks and shows zero-shot cross-modal transferability.

==> all_ast_ppl.tex <==
\begin{table*}[]
\centering
\begin{tabular}{c|rr|rl|rl|rl}
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{u2u}                           & \multicolumn{2}{c|}{t2u}       & \multicolumn{2}{c|}{u2t}       & \multicolumn{2}{c}{t2t}        \\ \hhline{=========}
Task           & \multicolumn{1}{l}{PPL} & \multicolumn{1}{l|}{CCS} & \multicolumn{1}{l}{PPL} & CCS  & \multicolumn{1}{l}{PPL} & CCS  & \multicolumn{1}{l}{PPL} & CCS  \\ \hhline{=========}
uLM+ASR+TTS+W-AST+TLM               & 25.05                   & 0.97                     & 27.18                   & \textbf{0.70} & 52.35                   & \textbf{0.81} & 77.59                   & 0.67 \\ \hline
uLM+ASR+TTS+S-AST+TLM                   & 25.18                   & 0.95                     & 31.75                   & 0.12 & 77.44                   & 0.17 & 80.32                  & 0.60 \\ \hline
uLM+TLM           & 26.31                   & 0.94                     & 47.93                   & 0.03 & 3098.63                   & 0.01 & 241.71                   & 0.20
\end{tabular}
\caption{Perplexity and CCS for W-AST, S-AST comparison. "u2t" means the prompt is unit and the continuation is text and so on. 
}\label{tab:ppl_all}
% I don't think we need to explain why we don't include PELM
\end{table*}

==> sections/7_discussion.tex <==
\section{Discussion}
% recent trend on TTS: fine-grain speech unit 
%LLM
In this work, we show that mixing speech units and text increase the cross-modal ability of the model. The additional text data enhance the model in different ways for downstream tasks. For SLUE-SA, the additional text data enable the model to zero-shot transfer between speech and text. For SLUE-SA we remove the output layer from the LM and attach a classification head so the model will always output a valid class. In the case of SLUE-NER, we observed a direct enhancement in performance, which we attribute to the additional text data helping the model generate better text. However, we note that fine-tuning strategies can produce different results, as demonstrated in~\cite{liu2021gpt}. we plan to investigate alternative fine-tuning approaches that can effectively handle the problem of trivial tasks and length mismatching when fine-tuning on text data. 
%We also observe a non-trivial transfer from speech to text in SLUE-NER similar to the result in~\cite{bapna2022mslam} on speech translation.

%ASR and TTS allows the model to learn shared representations but it won't enable the model to continue for prompts from the other modality. W-AST on the other hand helps the model in learning shared representations that can benefit both discriminative tasks e.g. SLUE-SA and generative task like speech/text continuation. 

We conducted our experiments on a medium scale (model with 350M parameters) model and evaluated it on a single-sentence basis for both automatic metrics and downstream tasks. The setup can be further extended by incorporating multi-lingual data, using multiple sentences, and large-scale models, etc. While our approach relies on the use of paired data, with a strong ASR system such as~\cite{radford2022robust} we can easily transcribe the speech into text. 

%The experiment result also suggested that our metric (CCS) correct reflect the performance on SLU downstream tasks. 

==> tables/pair_ppl.tex <==
\begin{table*}[h!]
\centering
\resizebox{2.2\columnwidth}{!}{
\begin{tabular}{c|c|rrr|rrr|rrr|rrr}
\multicolumn{2}{l|}{} & \multicolumn{3}{c|}{u2u}                           & \multicolumn{3}{c|}{t2u}       & \multicolumn{3}{c|}{u2t}       & \multicolumn{3}{c}{t2t}        \\ \hhline{==============}
ids & Task           & \multicolumn{1}{r}{PPL} & \multicolumn{1}{r}{CRA} & \multicolumn{1}{r|}{PELM} & \multicolumn{1}{r}{PPL} & CRA & \multicolumn{1}{r|}{PELM}  & \multicolumn{1}{r}{PPL} & CRA & \multicolumn{1}{r|}{PELM}  & \multicolumn{1}{r}{PPL} & CRA & \multicolumn{1}{r}{PELM}  \\ \hhline{==============}
(1) & \makecell{uLM+ASR+TTS}               & 24.92                   & 0.95   &                  & 30.34                   & \textbf{0.26} & & 97.67                   & \textbf{0.33} & & 91.37                   & 0.56& \\ \hline
(2) &uLM+S-AST                   & 25.36                   & 0.97      &       251.42        & 31.16                   & 0.10 & 306.27 & 94.91                   & 0.15 & 88.52 & 108.60                  & 0.44 & 47.05 \\ \hline
(3) & \makecell{uLM+ASR+TTS\\+S-AST}           & 25.09                   & 0.97   &        250.27          & 31.17                   & 0.11 &285.52 & 77.00                   & 0.11 & 96.18 & 81.49                   & 0.60&37.02 \\ \hhline{==============}
(4) & \makecell{uLM+ASR+TTS\\+W-AST+LM}               & 25.05                   & 0.97     &        246.54        & 27.18                   & \textbf{0.70} &154.85 & 52.35                   & \textbf{0.81} & 52.83 & 77.59                   & 0.67 & 34.64 \\ \hline
(5) & \makecell{uLM+ASR+TTS\\+S-AST+LM}                   & 25.18                   & 0.95   &    265.37              & 31.75                   & 0.12 & 306.54& 77.44                   & 0.17 & 97.39& 80.32                  & 0.60 & 34.92 \\ \hline
(6) & uLM+LM           & 26.31                   & 0.94         &       250.44     & 47.93                   & 0.03 & 907.08 & 3098.63                   & 0.01 & 1969.87 & 241.71                   & 0.20 & 21.64

\end{tabular}
}
\caption{Perplexity, CRA and PELM. "u2t" means the prompts are units and the continuations are text and so on.  
%For cross-modal scores (t2u, u2t), ASR+TTS have the best performance. It suggested that it helps the model to learn shared representations between speech and text. 
}%\label{tab:ppl_pair}
% I don't think we need to explain why we don't include PELM
\end{table*}

==> tables/pelm.tex <==
\begin{algorithm}
\caption{The procedure of PELM. We first sample continuation $x_{cont}$ from our model. Transcribe it if it is speech. Then we use an external LM to compute the perplexity. }\label{alg:pelm}
\begin{algorithmic}

\State $x_{cont} \sim P_{LM}(cont|prompt)$ 
\If{$x_{cont}$ is speech}
    \State $x_{cont} \gets transcribe(x_{cont})$
\EndIf
\State $PPL(x_{cont})=2^{\frac{\log P_{external}(x_{cont}|x_{prompt})}{\Vert x_{cont}\Vert}}$

\end{algorithmic}
\end{algorithm}


==> tables/table_unit.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|r|r|r|r|r}
 & \multicolumn{1}{|l|}{PPL} & \multicolumn{1}{l|}{CCS} & \multicolumn{1}{l|}{PELM} & \multicolumn{1}{l|}{SA} & \multicolumn{1}{l}{NER} \\ \hhline{======}
Basline   &                         &                         &                          & 0.46                        & 54.5                         \\ \hline
Ground truth   &                         &                         &           116.50               &                        &                          \\ \hline
HuBERT    & 5.22                    & \textbf{1.00}                    & 279.53                   & 0.51                        & 62.9                         \\ \hline
SP 10k    & 25.66                   & 0.96                    & \textbf{250.55}                   & \textbf{0.56}                        & \textbf{64.4} \\ \hline
SP 32k    & 57.44                   & 0.96                    & 265.14                   & 0.54                        & 62.5                        
\end{tabular}
}
\caption{We trained the LM on speech units to compare them (HuBERT, SP 10k, SP 32k) along with baseline~\cite{shon2022slue} and PELM on ground truth continuations.  \wh{TODO: PPLs are not comparable across units. let's put an asterik to PPL and add in caption that these number should not be directly compared}\kl{what is the purpose of having PPL in this table?}}\jc{Sorry this table is just to backup the commments. They are merged to the next table. }
%\label{tab:unit}
\end{table}
